RLlib Flow: Distributed Reinforcement Learning is a Dataflow Problem

Researchers and practitioners in the field of reinforcement learning (RL) frequently leverage parallel computation, which has led to a plethora of new algorithms and systems in the last few years. In this paper, we re-examine the challenges posed by distributed RL and try to view it through the lens of an old idea: distributed dataflow. We show that viewing RL as a dataflow problem leads to highly composable and performant implementations. We propose RLlib Flow, a hybrid actor-dataflow programming model for distributed RL, and validate its practicality by porting the full suite of algorithms in RLlib, a widely adopted distributed RL library. Concretely, RLlib Flow provides 2-9 code savings in real production code and enables the composition of multi-agent algorithms not possible by end users before. The open-source code is available as part of RLlib at https://github.com/ray-project/ray/tree/master/rllib.

==> figTex/archive/architecture.tex <==
\begin{figure}[h]
\includegraphics[width=0.98\linewidth]{figures/arch.pdf}
\vspace{-10pt}
\caption{High-level architecture diagram of \flowname, which is now part of \libname.}
\label{fig:arch}
\vspace{-10pt}
\end{figure}

==> figTex/archive/loc-library.tex <==
\begin{table}
\centering
\begin{tabular}{lcc}
    \toprule
            & Original & \flowname \\
    \midrule
    Base & 725 & 808 \\
    Model Base & 1496 & 1654 \\
    Env Base & 1720 & 3187 \\
    Optimizer Base & 3346 & -- \\
    Evaluation Base & 2590 & 4709 \\
    Policy Base & 2813 & 4831 \\
    Execution Base & -- & 2482 \\
    Agents Base & 1347 & 1830 \\
    Offline Base & 796 & 774 \\
    Total & 14752 &  20275 \\
    \bottomrule
\end{tabular}
\caption{Lines of code for original \libname vs our proposed \flowname-based \libname.}
\label{tab:loc-lib}
\tabspace
\end{table}

==> figTex/archive/maml-code.tex <==
\begin{figure}[t]
% https://docs.google.com/document/d/16CPp7yJbWqI1PbHlcvARNjxqZVGrMyd0l3GZ4zUsiFA/edit?usp=sharing
\centering
\includegraphics[width=0.9\linewidth]{figures/code/maml-code.pdf}
\vspace{-5pt}
\caption{Pseudocode for MAML in \flowname.}
\label{alg:maml-code}
\vspace{-10pt}
\end{figure}

==> figTex/archive/rllib-vs-spark.tex <==
% https://docs.google.com/drawings/d/11pJ7KkblxeipjecAqdBOk-iZUZid43dItsFt3Bd8TYA/edit
\begin{figure}[t]
\centering
% link: https://1drv.ms/p/s!Ah3_lLUfMlckjbtfFb8iw4nQmc6qtg?e=PMlppD
\includegraphics[width=.6\linewidth]{figures/rllib-vs-spark-small.pdf}
\caption{\revise{The throughput comparison between \flownamecap and Spark Streaming with PPO algorithm on CartPole-v0 environment.}}
% The running time is measured for one iteration on AWS m4.10xlarge CPU instances with 40 vCPUs and 10Gbps network each. \flowname achieves better training throughput and scalability against a Spark Streaming based implementation with up to 2.9\x faster speed.
\label{fig:rllib-spark}
\vspace{-10pt}
\end{figure}

==> figTex/archive/throughput-pong.tex <==
% https://docs.google.com/drawings/d/11pJ7KkblxeipjecAqdBOk-iZUZid43dItsFt3Bd8TYA/edit
\begin{figure}[t]
    \centering
    % link: https://1drv.ms/p/s!Ah3_lLUfMlckjbtqH49JqfLAko1eMQ?e=YsX2kL
    \includegraphics[width=0.97\linewidth]{figures/rllib-throughput-stack.pdf}
\figspace
\caption{Training throughput of \flowname based v.s. original \libname on Pong game with IMPALA.}
% The experiments are conducted on PongNoFrameSkip-v4 using IMPALA algorithm with AWS p3.16xlarge as the master and additional m4.16xlarge as actor workers. We achieve comparable performance across different versions of \libname. The red bars indicate the min and max throughput of three runs.
\label{fig:throughput}
\figspace
\end{figure}

==> figTex/archive/twotrainer.tex <==
\begin{figure}[h]
\includegraphics[width=\columnwidth]{figures/twotrainer.pdf}
\vspace{-18pt}
\caption{\libname dataflow diagram for concurrent multi-agent training of DQN and PPO agents in an environment.}
\label{fig:twotrainer}
\vspace{-5pt}
\end{figure}

==> figTex/throughput-tab.tex <==
\begin{table}[h]
% \tabspace
\vspace{-5pt}
\caption{Training throughput (samples/second) on different environments of original and our \flowname-based \libname. No additional overheads are introduced by \flowname.}
\vspace{5pt}
\centering
{\small
\begin{tabular}{lccc}
    \toprule
           & Workers (GPUs) & RLlib & \flowname  \\
    \midrule
    Pendulum & 2 (0) & 1.2K & 1.3K\\
    Breakout & 32 (4) & 4.5K & 4.1K \\
    Pong     & 200 (2) & 18.7K & 18.9K \\
    \bottomrule
\end{tabular}
}
% \tabspace

% Our new framework consistently achieves comparable or even better throughput than the original one.
\label{tab:throughput-tab}
\vspace{-5pt}
\end{table}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
